Spectral Continuity for Aperiodic Quantum Systems I. General Theory

How does the spectrum of a Schr\"odinger operator vary if the corresponding geometry and dynamics change? Is it possible to define approximations of the spectrum of such operators by defining approximations of the underlying structures? In this work a positive answer is provided using the rather general setting of groupoid $C^\ast$-algebras. A characterization of the convergence of the spectra by the convergence of the underlying structures is proved. In order to do so, the concept of continuous field of groupoids is slightly extended by adding continuous fields of cocycles. With this at hand, magnetic Schr\"odinger operators on dynamical systems or Delone systems fall into this unified setting. Various approximations used in computational physics, like the periodic or the finite cluster approximations, are expressed through the tautological groupoid, which provides a universal model for fields of groupoids. The use of the Hausdorff topology turns out to be fundamental in understanding why and how these approximations work. Corrigendum: A correct statement of Theorem 4 is provided. The change does not affect the main results.

==> RefCorrigendum.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%% September 27, 2016 %%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%                                                                  %%%%
%%%%       Spectral continuity for aperiodic quantum systems I.       %%%% 
%%%%                          General Theory                          %%%%
%%%%                                                                  %%%%
%%%%      Siegfried Beckus, Jean Bellissard, Giuseppe De Nittis,      %%%% 
%%%%                   Revised Version #7: 08/08/17                   %%%%
%%%%                                                                  %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{thebibliography}{9999}


\bibitem{BBD18} S.~Beckus, J.~Bellissard, G.~De~Nittis, ``{S}pectral continuity for aperiodic quantum systems {I}. {G}eneral Theory'', {\em J. Funct. Anal.}, {\bf 275}, 2917-2977, (2018).

\bibitem{Bl96} E.~Blanchard, ``D\'{e}formations de $C^\ast$-alg$\grave{e}$bres de Hopf'', {\em Bull. Sc. math.}, (\textbf{1}), no. 124, 141-215, (1996).

\bibitem{Det18} A.~Deitmar, ``On Haar Systems for Groupoids'', {\em Z. Anal. Anwend.}, {\bf 37}, 269-275, (2018).

\bibitem{Kas88} G.~G.~Kasparov, ``Equivariant {$KK$}-theory and the {N}ovikov conjecture'', {\em Invent. Math.}, {\bf 91}, 147-201, (1988).

\bibitem{Re80} J.~Renault, ``A Groupoid Approach to $C^{\ast}$-Algebras'', Lecture Notes in Math., {\bf 793}, Springer, Berlin, (1980).

\bibitem{We67} J.~Westman, ``Non transitive groupoid algebras'', Lecture notes, University of California at Irvine, (1967).

\bibitem{Wi16} D.~P.,~Williams, ``Haar Systems on Equivalent Groupoids'',  {\em Proc. Amer. Math. Soc.}, {\bf 3}, 1-8, (2016).

\end{thebibliography}

